Spin torque and force due to current for general spin textures

Non-adiabatic correction to spin transfer torque arising from fast-varying spin texture is calculated treating conduction electron fully quantum mechanically. The torque is non-local in space, and is shown to equivalent to a force (due to momentum transfer) acting on the center of mass of the texture. Another kind of force exists in the adiabatic regime, and is identified to be of topological origin. These forces are shown to be the counter reaction of electric transport properties, resistivity and Hall effect, respectively.

==> defs.tex <==
%\renewcommand{\half}{\frac{1}{2}} % defs for elsart class
\newcommand{\half}{\frac{1}{2}} % defs for other class
%%%%%%%%%%%%%%
\def\average#1{\left\langle {#1} \right\rangle}
\def\ddelo#1{\frac{d^2}{d #1^2}}
\def\ddel#1#2{\frac{d^2 #1}{d #2 ^2}}
\def\ddelpo#1{\frac{\partial^2}{\partial #1^2}}
\def\delo#1{\frac{d}{d #1}}
\def\delpo#1{\frac{\partial}{\partial #1}}
\def\deldo#1{\frac{\delta}{\delta #1}}
\def\del#1#2{\frac{d #1}{d #2}}
\def\delp#1#2{\frac{\partial #1}{\partial #2}}
\def\deld#1#2{\frac{\delta #1}{\delta #2}}
\def\vvec#1{\stackrel{{\leftrightarrow}}{#1}} %\def\vvec#1{\overleftrightarrow{#1}}
\def\vec2#1#2{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\def\vec3#1#2#3{\left(\begin{array}{c} #1 \\ #2 \\ #3 \end{array}\right)}
%%%%%%%%%%%%
\def\listitem#1{\begin{itemize}\item #1 \end{itemize}}
\newcommand{\lt}{\left}
\newcommand{\rt}{\right}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\adag}{{a^{\dagger}}}
\newcommand{\Area}{A}
\newcommand{\Av}{{\bm A}}
\newcommand{\AvEM}{{\bm A}_{\rm EM}}
\newcommand{\Aph}{A^{\phi}}
\newcommand{\Ath}{A^{\theta}}
\newcommand{\Aphv}{\Av^{\phi}}
\newcommand{\Athv}{\Av^{\theta}}
\newcommand{\Az}{{A^{z}}}
\newcommand{\Bv}{{\bm B}}
\newcommand{\Bz}{{B_z}}
\newcommand{\Bc}{B_{\rm c}}
\newcommand{\Bveff}{{\bm B}_{\rm eff}}
\newcommand{\Bve}{{\bm B}_{\rm e}}
%\newcommand{\chiz}{\chi^{z,{\rm r}}}
%\newcommand{\chipm}{\chi^{\pm,{\rm r}}}
\newcommand{\cdag}{{c^{\dagger}}}
\newcommand{\ckv}{c_{\kv}}
\newcommand{\ckvs}{c_{\kv\sigma}}
\newcommand{\dels}{{s_0}}
\newcommand{\dx}{{d^3 x}}
\newcommand{\DOS}{{\nu}}
\newcommand{\DOSV}{{N(0)}}
\newcommand{\DOSom}{{\nu_\omega}}
\newcommand{\ef}{{\epsilon_F}}
\newcommand{\eF}{{\epsilon_F}}
\newcommand{\ekv}{\epsilon_{\kv}}
\newcommand{\ekvs}{\epsilon_{\kv\sigma}}
\newcommand{\Ev}{{\bm E}}
\newcommand{\ev}{{\bm e}}
\newcommand{\evth}{{\bm e}_{\theta}}
\newcommand{\evph}{{\bm e}_{\phi}}
\newcommand{\evs}{{\bm n}}%{{\bm e}_{\rm s}}
\newcommand{\evsz}{{\evs}_0}
\newcommand{\evsph}{{\bm e}_{{\rm s}\phi}}
\newcommand{\evz}{{\bm e}_{z}}
\newcommand{\fl}{{\eta}}
\newcommand{\fltil}{\tilde{\eta}}
\newcommand{\flitil}{\tilde{\fl_{\rm I}}}
\newcommand{\flrtil}{\tilde{\fl_{\rm R}}}
\newcommand{\fli}{{\fl_{\rm I}}}
\newcommand{\flr}{{\fl_{\rm R}}}
\newcommand{\fkvs}{f_{\kv\sigma}}
\newcommand{\fo}{{f(\omega)}}
\newcommand{\fpo}{{f'(\omega)}}
%\newcommand{\fomega}{{\omega}}
\newcommand{\fpin}{{f_{\rm pin}}}
\newcommand{\fe}{{f_{\rm e}}}
\newcommand{\Fe}{{F_{\rm e}}}
\newcommand{\Fev}{{\Fv_{\rm e}}}
\newcommand{\Fena}{{F_{\rm e}^{\rm na}}}
\newcommand{\Fv}{{\bm F}}
\newcommand{\gv}{{\bm g}}
\newcommand{\gr}{g^{\rm r}}
\newcommand{\ga}{g^{\rm a}}
\newcommand{\gless}{g^{<}}
\newcommand{\Gr}{G^{\rm r}}
\newcommand{\Ga}{G^{\rm a}}
\newcommand{\Gless}{G^{<}}
\newcommand{\ggtr}{g^{>}}
\newcommand{\gap}{\Delta_{\rm sw}}
\newcommand{\gammap}{\gamma_{+}}
\newcommand{\gammam}{\gamma_{-}}
\newcommand{\hf}{\frac{1}{2}}
%\newcommand{\half}{\frac{1}{2}}
\newcommand{\HA}{{H_{A}}}
\newcommand{\HB}{H_{B}}
\newcommand{\He}{H_{\rm e}}
\newcommand{\Heff}{H_{\rm eff}}
\newcommand{\Hem}{H_{\rm EM}}
\newcommand{\Hex}{H_{\rm ex}}
\newcommand{\Himp}{H_{\rm imp}}
\newcommand{\HR}{{H_{\rm R}}}
\newcommand{\Hs}{{H_{\rm S}}}
\newcommand{\Hsf}{{H_{\rm sf}}}
\newcommand{\Hst}{{H_{\rm ST}}}
\newcommand{\hbarinv}{\frac{1}{\hbar}}
\renewcommand{\Im}{{\rm Im}}
\newcommand{\intinf}{\int_{-\infty}^{\infty}}
\newcommand{\intom}{\int \frac{d\omega}{2\pi}}
\newcommand{\intx}{\int {d^3x}}
\newcommand{\iv}{\bm{i}}
\newcommand{\Iv}{\bm{I}}
\newcommand{\Js}{{J_{\rm s}}}
\newcommand{\js}{j_{\rm s}}
\newcommand{\jsc}{{j_{\rm s}^{\rm c}}}
\newcommand{\jsv}{\bm{j}_{\rm s}}
\newcommand{\jc}{j_{\rm c}}
\newcommand{\jci}{{{j}_{\rm c}^{\rm i}}}
\newcommand{\jce}{{{j}_{\rm c}^{\rm e}}}
\newcommand{\jatil}{{\tilde{j}_{\rm a}}}
\newcommand{\jctil}{{\tilde{j}_{\rm c}}}
\newcommand{\jcitil}{{\tilde{j}_{\rm c}^{\rm i}}}
\newcommand{\jcetil}{{\tilde{j}_{\rm c}^{\rm e}}}
\newcommand{\jtil}{{\tilde{j}}}
\newcommand{\jv}{\bm{j}}
\newcommand{\kB}{{k_B}}
\newcommand{\kb}{{k_B}}
\newcommand{\kv}{{\bm k}}
%\newcommand{\kvp}{{\kv}_{\perp}}
\newcommand{\kvp}{{\kv}'}
\newcommand{\kpq}{{k+\frac{q}{2}}}
\newcommand{\kmq}{{k-\frac{q}{2}}}
\newcommand{\kvpq}{{\kv}+\frac{\qv}{2}}
\newcommand{\kvmq}{{\kv}-\frac{\qv}{2}}
\newcommand{\kvppq}{{\kvp}+\frac{\qv}{2}}
\newcommand{\kvpmq}{{\kvp}-\frac{\qv}{2}}
\newcommand{\kf}{{k_F}}
\newcommand{\kF}{{k_F}}
\newcommand{\kfpm}{{k_{F\pm}}}
\newcommand{\kfmp}{{k_{F\mp}}}
\newcommand{\kom}{{k_\omega}}
\newcommand{\Kp}{{K_\perp}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\lams}{{\lambda_{\rm s}}}
\newcommand{\lamv}{{\lambda_{\rm v}}}
\newcommand{\lamz}{{\lambda_{0}}}
\newcommand{\Le}{{L_{\rm e}}}
\newcommand{\Lb}{{L_{\rm B}}}
\newcommand{\Ldw}{{L_{\rm dw}}}
\newcommand{\Ls}{{L_{\rm S}}}
\newcommand{\Lsw}{{L_{\rm sw}}}
\newcommand{\Lswdw}{{L_{\rm sw-dw}}}
\newcommand{\Linv}{{\frac{1}{L}}}
\newcommand{\mv}{{\bm m}}
\newcommand{\Mv}{{\bm M}}
\newcommand{\Mw}{{M_{\rm w}}}
\newcommand{\mus}{{g\mu_{B}}}
\newcommand{\muB}{\mu_B}
\newcommand{\Ne}{N_{\rm e}}
\newcommand{\nv}{{\bm n}}
\newcommand{\nimp}{n_{\rm imp}}
\newcommand{\nvortex}{n_{\rm v}}
\newcommand{\nz}{{n}_0}
\newcommand{\om}{{\omega}}
\newcommand{\Omegatil}{{\tilde{\Omega}}}
\newcommand{\Omegap}{{{\Omega'}}}
\newcommand{\Omegaptil}{{\tilde{\Omegap}}}
\newcommand{\Omz}{{{\Omega_0}}}
\newcommand{\ompOmz}{{\omega+\frac{\Omz}{2}}}
\newcommand{\ommOmz}{{\omega-\frac{\Omz}{2}}}
\newcommand{\phiz}{{\phi_0}}
\newcommand{\PhiB}{{\Phi_{\rm B}}}
\newcommand{\Ptil}{{\tilde{P}}}
\newcommand{\pv}{{\bm p}}
\newcommand{\qv}{{\bm q}}
\newcommand{\qtil}{{\tilde{q}}}
\renewcommand{\Re}{{\rm Re}}
\newcommand{\rhow}{{\rho_{\rm w}}}
\newcommand{\rhos}{{\rho_{\rm S}}}
\newcommand{\rhoS}{{\rho_{\rm S}}}
\newcommand{\rhoxy}{{\rho_{xy}}}
\newcommand{\RS}{{R_{\rm S}}}
\newcommand{\Rw}{{R_{\rm w}}}
\newcommand{\rv}{{\bm r}}
\newcommand{\Rv}{{\bm R}}
\newcommand{\sigmav}{{\bm \sigma}}
%\newcommand{\sigmavtil}{\tilde{\bm \sigma}}
\newcommand{\se}{{s}}
\newcommand{\sev}{{\bm \se}}
\newcommand{\sgn}{{\rm sgn}}
\newcommand{\sz}{{s}_0}
\newcommand{\sv}{{{\bm s}}}
\newcommand{\seth}{{\se}_\theta}
\newcommand{\seph}{{\se}_\phi}
\newcommand{\sez}{{\se}_z}
\newcommand{\svtil}{\tilde{\bm s}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\stilz}{\stil_{z}}
\newcommand{\stilpara}{\stil_{\parallel}}
\newcommand{\stilperp}{\stil_{\perp}}
\newcommand{\Simpv}{{{\bm S}^{\rm i}}}
\newcommand{\Simp}{{S^{\rm i}}}
\newcommand{\Sh}{{\hat {S}}}
\newcommand{\Svh}{{\hat {\Sv}}}
\newcommand{\Sv}{{{\bm S}}}
\newcommand{\Svz}{{{\bm S}_0}}
\newcommand{\sumx}{{\int \frac{d^3x}{a^3}}}
\newcommand{\sumk}{{\sum_{k}}}
\newcommand{\sumkv}{{\sum_{\kv}}}
\newcommand{\sumom}{\int\frac{d\omega}{2\pi}}
\newcommand{\sumOm}{\int\frac{d\Omega}{2\pi}}
\newcommand{\sumomOm}{\int\frac{d\omega}{2\pi}\int\frac{d\Omega}{2\pi}}
%\newcommand{\sumom}{{\sum_{\omega}}}
\newcommand{\sumqv}{{\sum_{\qv}}}
\newcommand{\thickness}{{d}}
\newcommand{\thetaz}{{\theta_0}}
\newcommand{\tr}{{\rm tr}}
\newcommand{\Tc}{{T_{C}}}
\newcommand{\Torqv}{{\bm \tau}}
\newcommand{\torque}{{\tau}}
\newcommand{\torquev}{{\bm \torque}}
\newcommand{\Torquev}{{\bm \tau}}
\newcommand{\torqueve}{{\torquev_{\rm e}}}
\newcommand{\torquee}{{\torque_{\rm e}}}
\newcommand{\tautil}{{\tilde{\tau}}}
\newcommand{\taup}{\tau_{+}}
\newcommand{\taum}{\tau_{-}}
\newcommand{\tauw}{\tau_{\rm w}}
\newcommand{\tausf}{\tau_{\rm sf}}
\newcommand{\thetast}{\theta_{\rm st}}
\newcommand{\ttil}{{\tilde{t}}}
\newcommand{\tz}{{t_0}}
\newcommand{\vc}{{v^{\rm c}}}
\newcommand{\ve}{{v_{\rm e}}}
\newcommand{\vv}{\bm{v}}
\newcommand{\vsv}{{\vv_{\rm s}}}
\newcommand{\vf}{{v_F}}
\newcommand{\vimp}{v_{\rm imp}}
\newcommand{\vi}{{v_{\rm i}}}
\newcommand{\vtil}{{{v_0}}}
%\newcommand{\vtil}{{\tilde{v}}}
\newcommand{\Vpin}{{V}_{\rm pin}}
\newcommand{\Vinv}{\frac{1}{V}}
\newcommand{\vz}{{v_0}}
\newcommand{\Vz}{{V_0}}
\newcommand{\Vztil}{{\tilde{V_0}}}
\newcommand{\Ws}{{W_{\rm S}}}
\newcommand{\Xtil}{{\tilde{X}}}
\newcommand{\xv}{{\bm x}}
\newcommand{\Xv}{{\bm X}}
\newcommand{\xvp}{{\bm x}_{\perp}}
\newcommand{\xw}{{z}}
\newcommand{\Xz}{{X_0}}
\newcommand{\Zs}{Z_{\rm S}}
\newcommand{\ztil}{u}%{\tilde{\xw}}

